Practical Mutation Testing at Scale

Mutation analysis assesses a test suite's adequacy by measuring its ability to detect small artificial faults, systematically seeded into the tested program. Mutation analysis is considered one of the strongest test-adequacy criteria. Mutation testing builds on top of mutation analysis and is a testing technique that uses mutants as test goals to create or improve a test suite. Mutation testing has long been considered intractable because the sheer number of mutants that can be created represents an insurmountable problem -- both in terms of human and computational effort. This has hindered the adoption of mutation testing as an industry standard. For example, Google has a codebase of two billion lines of code and more than 500,000,000 tests are executed on a daily basis. The traditional approach to mutation testing does not scale to such an environment. To address these challenges, this paper presents a scalable approach to mutation testing based on the following main ideas: (1) Mutation testing is done incrementally, mutating only changed code during code review, rather than the entire code base; (2) Mutants are filtered, removing mutants that are likely to be irrelevant to developers, and limiting the number of mutants per line and per code review process; (3) Mutants are selected based on the historical performance of mutation operators, further eliminating irrelevant mutants and improving mutant quality. Evaluation in a code-review-based setting with more than 24,000 developers on more than 1,000 projects shows that the proposed approach produces orders of magnitude fewer mutants and that context-based mutant filtering and selection improve mutant quality and actionability. Overall, the proposed approach represents a mutation testing framework that seamlessly integrates into the software development workflow and is applicable up to large-scale industrial settings.

==> figures/comparison.tex <==
\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color2}{rgb}{0.556862745098039,0.729411764705882,0.258823529411765}
\definecolor{color3}{rgb}{0.856862745098039,0.729411764705882,0.258823529411765}

\pgfplotsset{scaled y ticks=false}
\begin{figure}[htb]
\centering
  \resizebox{0.5\textwidth}{!}{
  \begin{tikzpicture}
    \begin{axis}[
        ymode=log,log basis y=10,
        legend style={at={(0.5,-0.2)}, anchor=north,legend columns=2,draw=none},
        legend style={/tikz/every even column/.append style={column sep=0.5cm}},
        ylabel={\textsc{Mutants}},
        ylabel near ticks,
        xlabel={\textsc{Diff}},
        axis x line=none,
        ytick pos=left,
        ymin=1,
        bar width=10pt,
      ]
      \addplot[color=color0, only marks] table [x=Diff, y=Classical, col sep=comma] {figures/classic_vs_google_comparison.csv};
      \addplot[color=color1, only marks, mark=square*] table [x=Diff, y=Google, col sep=comma] {figures/classic_vs_google_comparison.csv};
      \legend{classical,suppressed}
    \end{axis}
  \end{tikzpicture}
  }
  \caption{Mutants generated by classical vs Google's mutagenesis. Notice the classical approach yields up to 50'000 while suppressed up to 1'000 mutants.}
  \label{fig:comparison}
\end{figure}


==> figures/fitness.tex <==








\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color2}{rgb}{0.556862745098039,0.729411764705882,0.258823529411765}
\definecolor{color3}{rgb}{0.856862745098039,0.729411764705882,0.258823529411765}


==> figures/opdist.tex <==
\begin{figure}[H]
  \begin{tikzpicture}
   \tikzset{ lines/.style={draw=none}, }
   \pie[rotate=180,explode = {0.2},text=pin,after number=,
      color={color1!70, color2!70, color0!70, color3!70, color4!70},
      every only number node/.style={text=black},style={lines}
    ]
    {73.25/SBR, 16.05/UOI, 4.38/ROR, 4.07/LCR, 2.25/AOR}
  \end{tikzpicture}
  \caption{Overall mutant ratio by mutation operator}
  \label{fig:opdist}
\end{figure}


==> figures/survival.tex <==











==> sections/future_work.tex <==
%\section{Future Work}
\label{future_work}

For future work,
% we plan to replace the proposed mutation context scheme with a
%more generic representation. For example, we plan to experiment with different
%embeddings, such as Code2Vec~\cite{code2vec}, for AST nodes under mutation, and
%compare how different normalizations of the embedding space affect the results.
%
%Furthermore,
we plan to investigate the long-term effects of mutation testing on
developer behavior when writing tests. We conjecture that developers exposed to
mutation testing over a long period of time get accustomed to these test goals
and proactively write more tests prior to sending the code for review,
thus ensuring better test quality and saving review time.

%Finally, we plan to analyze fault coupling by looking into production bugs and
%testing whether, if mutation testing had been run on the diff introducing the
%bug, would such a mutant be reported that if fixed at the time of code review,
%it would prevent the bug from being submitted to the repository in the first
%place.

